Adversarial attacks on hybrid classical-quantum Deep Learning models for Histopathological Cancer Detection

We present an effective application of quantum machine learning in histopathological cancer detection. The study here emphasizes two primary applications of hybrid classical-quantum Deep Learning models. The first application is to build a classification model for histopathological cancer detection using the quantum transfer learning strategy. The second application is to test the performance of this model for various adversarial attacks. Rather than using a single transfer learning model, the hybrid classical-quantum models are tested using multiple transfer learning models, especially ResNet18, VGG-16, Inception-v3, and AlexNet as feature extractors and integrate it with several quantum circuit-based variational quantum circuits (VQC) with high expressibility. As a result, we provide a comparative analysis of classical models and hybrid classical-quantum transfer learning models for histopathological cancer detection under several adversarial attacks. We compared the performance accuracy of the classical model with the hybrid classical-quantum model using pennylane default quantum simulator. We also observed that for histopathological cancer detection under several adversarial attacks, Hybrid Classical-Quantum (HCQ) models provided better accuracy than classical image classification models.

==> comment.tex <==
---------------COMMENT Start---------Keep a different section like literature Review to explain different types of attacks no relevance in introduction. Need to improve the introduction with soft intro of adversarial attacks, maybe an example of some paper, where adversarial attack is shown dangerous to medical field, discussing why the need of mitigate adversarial attacks. \\

Since only Boundary attack and gradient attack is used in the study its better to include those two only.\\ 
Note :- Once the draft is done the last paragraph of Introduction should include about the section below like section 2 discusses about methods used in our study include 1-2 line as what to expect like architecture, section 3 results and section 4 conclusion ------COMMENT END----- \\

% table is table 1 examples of adversarial attacks
\\ ------COMMENT START-------TABLE NOt referred anywhere------COMMENT END ----- \\

% figure : 1 contains types of attacks sued in our research

\\ ------COMMENT START------- Figure not discussed 
 anywhere------COMMENT END ----- \\
